Tasting the SU(5) nature of supersymmetry at the LHC

We elaborate on a recently found SU(5) relation confined to the up-(s)quark flavour space, that remains immune to large quantum corrections up to the TeV scale. We investigate the possibilities opened by this new window on the GUT scale in order to find TeV-scale SU(5) tests realizable at the LHC. These SU(5) tests appear as relations among observables involving either flavour violation or chirality flip in the up-(s)quark sector. The power of these tests is systematically evaluated using a frequentist, p-value based criterion. SU(5) tests in the Heavy supersymmetry (SUSY), Natural supersymmetry and Top-charm supersymmetry spectra are investigated. The latter scenario features light stops and scharms and is well-motivated from various five-dimensional constructions. A variety of SU(5) tests is obtained, involving techniques of top polarimetry, charm-tagging, or Higgs detection from SUSY cascade decays. We find that O(10) to O(100) events are needed to obtain 50% of relative precision at 3-sigma significance for all of these tests. In addition, we propose a set of precision measurements in ultraperipheral collisions in order to search for the flavour-changing dipole operators of Heavy supersymmetry.

==> numerics_SU5/numerics_SU5_2.0.tex <==
%!TEX root=paper.tex

% =================================================
\section{Persistence of the $SU(5)$ relation at low-energy} 
\label{Sec:Numerics}

In the previous section,  we saw that the $SU(5)$ relation $a_u\approx a_u^t$ remains qualitatively at low scale. 

Here we evaluate precisely the low-energy discrepancy $\epsilon^{\rm irr}$ induced by the RG flow. This discrepancy constitutes an irreducible bound on the precision at which one can test the $a_u\approx a_u^t $ relation. 

We present the results for a given benchmark of the MSSM. 
The qualitative study of the RG flow and further studies in the MSSM parameter space make clear that 




In this Section we would like to quantify numerically how much the relation of our interest Eq.\ \eqref{Eq:TrilinearUp}, is spoiled when evolved from the GUT scale down to the low SUSY scale.
To do so, we use the spectrum calculator {\tt SPhenoMSSM}, which is obtained by making use of the interface between the Mathematica package {\tt SARAH} \cite{Staub:2013tta} and the public code {\tt SPheno} \cite{Porod:2003um}. 
%using the interface between the Spectrum Generator Generators Sarah (v4.2.3 see \cite{Staub:2013tta}) and the well known code SPheno (v3.3.2 see \cite{Porod:2003um}).
{\tt SPhenoMSSM} solves the RGEs of the MSSM at two-loop order using a general flavour-violation pattern and hence, allows to compute low-scale mass spectra from GUT defined boundary conditions.
Note that this numerical study was done using the Supersymmetry Paramater Analysis convention (SPA see \cite{AguilarSaavedra:2005pw}) which in particular, imply that all low scale SSB parameters are given in the $\overline{\textrm{DR}}$ scheme at $M_{\textrm{SUSY}}$=1TeV.
Precisely, we study how high was the asymmetry on the up trilinear couplings normalized to the norm of the up squarks matrix, i.e :
\begin{equation}
	\mathcal{A}_{ij} ~=~ \frac{\left|(a_{u})_{ij}-(a_{u})_{ji}\right|}{\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} } }\,, \quad i\neq j\
\end{equation}
when varying the off diagonals elements of the up and down trilinear couplings at $M_{\textrm{GUT}}$ i.e $\mathcal{A}_{ij}=f((a_u)_{23},(a_d)_{32})$ where $(a_u)_{ij},(a_d)_{ij}$ are understood to be given at $M_{\textrm{GUT}}$.
A priori, there are three sectors to be investigated i.e $\mathcal{A}_{12},\mathcal{A}_{13}$ and $\mathcal{A}_{23}$. However the (1,2) and (1,3) sectors are too constrained by the requirement that one should not get negative physical masses in the low scale spectrum and that loop corrections should not lead the CKM matrix to be outside the experimental range, therefore in the following only $A_{23}$ will be considered.
We implement SU(5)-like boundaries conditions i.e $M^2_\mathrm{Q}, M^2_\mathrm{U}$, $M^2_\mathrm{E}$ are unified in $M^2_{\mathbf{10}}$ and $M^2_\mathrm{L}$, $M^2_\mathrm{D}$ in $M^2_{\bar{\mathbf{5}}}$.
We also choose for simplicity, at the GUT scale, a common Higgs mass i.e $M_H \equiv M_Hu=M_Hd$ and a common Gauginos mass noted $M_{1/2}$.
Finally we neglect all complex phases but the one introduced by the CKM matrix.
The benchmark point we take is given in table \ref{Num:Tab:BenchmarkPoint}.

\begin{table}
	\begin{center}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $\left(M^2_{\bold{10}}\right)_{i,j}$ & j=1       & j=2        & j=3      \\
				  \hline
				                                           i=1  & $(1000)^2$& 0          & 0        \\
				  \hline
				                           			       i=2  & 0         & $(3270)^2$ & $(557)^2$\\ 
				  \hline
				                            		       i=3  & 0         & $(557)^2$  & $(1550)^2$\\ 
				  \hline  
			\end{tabular}
			\hspace{0.5cm}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $\left(M^2_{\bold{\bar{5}}}\right)_{i,j}$ & j=1       & j=2        & j=3      \\
				  \hline
				                                           i=1  & $(860)^2$ & 0         & 0         \\
				  \hline
				                           			       i=2  & 0         & $(374)^2$ & 0         \\ 
				  \hline
				                            		       i=3  & 0         & 0         & $(412)^2$ \\ 
				  \hline  
			\end{tabular} 
			\vspace{0.5cm} \\
			\begin{tabular}{|l|l|l|l|} 
				
				  \hline
				  $a_u $ & j=1       & j=2       & j=3      \\
				  \hline
				   i=1   & 0         & 0         & 0         \\
				  \hline
				   i=2   & 0         & 0         & $(a_u)_{32}$\\ 
				  \hline
				   i=3   & 0         & $(a_u)_{23}$& -1500      \\ 
				  \hline  
			\end{tabular} 
			\hspace{0.5cm}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $a_d $ & j=1       & j=2       & j=3      \\
				  \hline
				   i=1   & 0         & 0         & 0         \\
				  \hline
				   i=2   & 0         & 0         & $(a_d)_{32}$\\ 
				  \hline
				   i=3   & 0         & $(a_d)_{23}$& 400      \\ 
				  \hline  
			\end{tabular}
			\hspace{0.5cm}
		\begin{tabular}{|l|} 
		 	\hline
		 	 $(M_{1∕2})^2=(1000)^2$ \\
		 	\hline 
			 $(M_{H})^2=(1000)^2$  \\
			\hline 
			 $\mathrm{sign}(\mu)=+1$ \\
		 	\hline
		\end{tabular}
	\end{center}
\caption{GUT-defined soft breaking parameters: All masses and trilinear couplings are given in GeV. \label{Num:Tab:BenchmarkPoint}}
\end{table}

%Placing 1: Figures are at the end of the section but not on the same page!!%%%%%%%%%%%%%%%

	\begin{figure}[b]%\RawFloats
		\centering
	   \includegraphics[scale=0.60]{numerics_SU5/figures/SmallTanB/LowTanB.pdf}
	\caption{\label{Num:Pic:LowTanB}Low $\tan \beta$ regime: The thick black lines represent the isolines of $\mathcal{A}_{2,3}$ expressed in percentages of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} }$. The blue dashed lines and the red dashed-dotted lines  are the 2$\sigma$  exclusion bands on $\Delta M_\mathrm{Bs}$ and $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ respectively. The grey area represents the space which is excluded once all constraints are taken into account.}
	\end{figure}
		
	\begin{figure}[t]
		\centering
		\includegraphics[scale=0.60]{numerics_SU5/figures/HighTanB/HighTanB.pdf}
	\caption{\label{Num:Pic:HighTanB}High $\tan \beta$ regime: Same as figure \ref{Num:Pic:LowTanB}, the green dotted line is the lower bound of the 2$\sigma$ exclusion band on $\mathrm{BR}(b \rightarrow s \gamma)$.} 
	\end{figure}

We have analyzed the asymmetry in a low $\tan(\beta) \sim 10$ and a high $\tan(\beta) \sim 40$ regime.
In order to clarify which region of parameter space is allowed experimentally, we also take into account several low energy flavor constraints among which the $B_s$ mesons oscillation frequency $\Delta M_{Bs}$ and the ratio of the K mesons mixing parameter normalized to the Standard Model value $\epsilon_K/\epsilon_K^{\textrm{SM}}$.
A full list of the constraints we included in this analysis, with theirs 2$\sigma$ uncertainties, can be found in table \ref{Num:Tab:ListConstraints}.

%Constraint table: With definitions of the constraints ---> Widder table.
\begin{table}
\begin{center}
\begin{tabular}{|l|}
\hline
	 $\Delta M_{Bs} = (17.76 \pm 3.37)$ $\mathrm{ps}^{-1}$ \\
\hline
	 $\epsilon_K/\epsilon_K^{\textrm{SM}} = (1 \pm 0.25)$ \\
\hline
	 $\mathrm{BR}(B^0_s\rightarrow \mu \mu) = (3.12 \pm 2.08)\times 10^{-9}$ \\
\hline
	 $\mathrm{BR}(b \rightarrow s \gamma) = (355 \pm 68)\times 10^{-6} $ \\
\hline	
	 $\mathrm{BR}(\tau \rightarrow \mu \gamma) < 4.5\times 10^{-8}$ \\
\hline
\end{tabular}
\end{center}
\vspace{0.2cm}
\caption{Low energy constraints used in the numerical analysis.\label{Num:Tab:ListConstraints}}	
\end{table}
	

%Constraint table: Without definitions of the constraints.


%\begin{tabular}{|l|}
%\hline
%	 $\Delta M_{Bs} = (17.76 \pm 3.37)$ $\mathrm{ps}^{-1}$ \\
%\hline
%	 $\epsilon_K/\epsilon_K^{\textrm{SM}} = (1 \pm 0.25)$ \\
%\hline
%	 $\mathrm{BR}(B^0_s\rightarrow \mu \mu) = (3.12 \pm 2.08)\times 10^{-9}$ \\
%\hline
%	 $\mathrm{BR}(b \rightarrow s \gamma) = (355 \pm 68)\times 10^{-6} $ \\
%\hline	
%	 $\mathrm{BR}(\tau \rightarrow \mu \gamma) < 4.5\times 10^{-8}$  \\
%\hline		
%\end{tabular}


%Constraint table: liste a puce, Peux etre pas top niveau presentation.


%\begin{enumerate}
%	\item[$\rightarrow$] $\Delta M_{Bs} = (17.76 \pm 3.37)$ $\mathrm{ps}^{-1}$: The $B_s$ mesons oscillation frequency. 
%	\item[$\rightarrow$] $\epsilon_K/\epsilon_K^{\textrm{SM}} = (1 \pm 0.25)$: The ratio of the K mesons mixing parameter normalized to the value of the Standard Model. 
%	\item[$\rightarrow$] $\mathrm{BR}(B^0_s\rightarrow \mu \mu) = (3.12 \pm 2.08)\times 10^{-9}$: The $B^0_s\rightarrow \mu \mu$ decay branching ratio.
%	\item[$\rightarrow$] $\mathrm{BR}(b \rightarrow s \gamma) = (355 \pm 68)\times 10^{-6} $: The $b \rightarrow s \gamma$ decay branching ratio.
%	\item[$\rightarrow$] $\mathrm{BR}(\tau \rightarrow \mu \gamma) < 4.5\times 10^{-8}$: The lepton number violating decay branching ratios of $\tau \rightarrow \mu \gamma$.
%\end{enumerate}
For each constraint, we make the quadratic sum of the experimental and theoretical errors.
We take the central values and experimental errors from the latest 2012 Heavy Flavor Collaboration Averaging Group report (see \cite{Amhis:2012bh}) and the theoretical errors from the following references (\cite{Misiak:2006zs}, \cite{Ball:2006xx}, \cite{Brod:2010mj}).
Moreover, we take into account the lightest higgs mass which we have assumed to correspond to the recently discovered scalar at the LHC. For its mass, we take the latest ATLAS central value 125.36$\pm$0.41(sys+stat) GeV see (\cite{Aad:2014aba}) quadratically summed with a theoretical error of $\pm$3 GeV.
The results are presented in fig \ref{Num:Pic:LowTanB} for the low $\tan \beta$ regime and in fig \ref{Num:Pic:HighTanB} for the high $\tan \beta$ regime.
On both figures, the thick black isolines represent the assymetry $\mathcal{A}_{2,3}$ expressed in percentage of $\sqrt{{\rm Tr}\mathcal{M}^2_{\tilde{u}}}$.
Note that we need to restrict this analysis to $ |(a_u)_{23}| < 600$ GeV, $|(a_d)_{23}| < 400$ GeV to avoid tachyons in the low scale spectrum, in particular the presence of tachyons in the spectrum depends critically on $(a_d)_{23}$.
We represent by colored lines the $2 \sigma$ exclusion band of the constraints when appropriate and by grey areas the excluded parameters space once all constraints are taken into account. 
In both regimes, $\mathrm{BR}(\tau \rightarrow \mu \gamma)$ never exceed the upper experimental value. We also manage to get a high and constant higgs mass ($m_h\sim$ 124 GeV) over the parameters range, especially due to the large negative top a-term ($a_t=-1500$ GeV).
In the low $\tan \beta$ regime, $\mathrm{BR}(b \rightarrow s \gamma)$ is kept within the $2\sigma$ exclusion band whereas this constraint is more severe for $\tan \beta \sim 40$, a part of the parameter space being excluded by it.
In the low $\tan \beta$ regime $\epsilon_K/\epsilon_K^{\textrm{SM}}$ is kept within the 1$\sigma$ band, due to the absence of complex phases in the soft terms, whereas in the high $\tan \beta$ regime, the supersymmetric contributions to $\epsilon_K$ are strongly suppressed, 
thus leading to $\epsilon_K/\epsilon_K^{\textrm{SM}} \sim 1$.
In any case, $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ and $\Delta M_{Bs}$ set the strongest constraints over the scanned parameter space (cf figs \ref{Num:Pic:LowTanB} and \ref{Num:Pic:HighTanB}).
To conclude, we see that the assymetry never exceed a few percents of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}}}$ which confirm that the relation of our interest \ref{Eq:TrilinearUp} is indeed well preserved when running from $M_\textrm{GUT}$ down to $M_\textrm{SUSY}$ thus allowing to treat it as a theoretical uncertainty.






	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Placing 2: Figures are gathered on the same page at the end of the section. Comes at the prize of half a page blank!%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%	\begin{figure}[p]%\RawFloats
%		\centering
%	   
%	   \includegraphics[scale=0.60]{numerics_SU5/figures/SmallTanB/LowTanB.pdf}
%	\caption{\label{Num:Pic:LowTanB}Low $\tan \beta$ regime: The thick black lines represents the isolines of $\mathcal{A}_{2,3}$ expressed in percentages of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} }$.  The  blue dashed lines and the red dashed-dotted lines  are the 2$\sigma$  exclusions bands on $\Delta M_\mathrm{Bs}$ and $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ respectively. The grey area represents the space which is excluded once all constraints are taken into account.}
%	
%		\centering
%		
%		\includegraphics[scale=0.60]{numerics_SU5/figures/HighTanB/HighTanB.pdf}
%	\caption{\label{Num:Pic:HighTanB}High $\tan \beta$ regime: Same as figure \ref{Num:Pic:LowTanB}, the green dotted line is the lower bound of the 2$\sigma$ exclusion band on $\mathrm{BR}(b \rightarrow s \gamma)$.} 
%		
%	\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\FloatBarrier

==> numerics_SU5/numerics_SU5_2_Save.0.tex <==
%!TEX root=paper.tex

% =================================================
\section{Persistence of the \texorpdfstring{$SU(5)$}{SU5} relation at low-energy} 
\label{Sec:Numerics}

In this Section we would like to quantify numerically how much our the relation of our interest, Eq.\ \eqref{Eq:TrilinearUp}, is spoiled when evolved from the GUT scale down to the low SUSY scale.
To do so, we use the spectrum calculator {\tt SPhenoMSSM}, which is obtained by making use of the interface between the Mathematica package {\tt SARAH} \cite{Staub:2013tta} and the public code {\tt SPheno} \cite{Porod:2003um}. 
%using the interface between the Spectrum Generator Generators Sarah (v4.2.3 see \cite{Staub:2013tta}) and the well known code SPheno (v3.3.2 see \cite{Porod:2003um}).
{\tt SPhenoMSSM} solves the RGEs of the MSSM at two-loop order using a general flavour-violation pattern and hence, allows to compute low-scale mass spectra from GUT defined boundary conditions.
Note that this numerical study was done using the Supersymmetry Paramater Analysis convention (SPA see \cite{AguilarSaavedra:2005pw}) which in particular, imply that all low scale SSB parameters are given in the $\overline{\textrm{DR}}$ scheme at $M_{\textrm{SUSY}}$=1TeV.
Precisely, we study how high was the asymmetry on the up trilinear couplings normalized to the norm of the up squarks matrix, i.e.
\begin{equation}
	\mathcal{A}_{ij} ~=~ \frac{\left|(a_{u})_{ij}-(a_{u})_{ji}\right|}{\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} } }\,, \quad i\neq j\, .
\end{equation}
when varying the off diagonal elements of the up and down trilinear couplings at $M_{\textrm{GUT}}$ i.e $\mathcal{A}_{ij}=f((a_u)_{23},(a_d)_{32})$ where $(a_u)_{ij},(a_d)_{ij}$ are understood to be given at $M_{\textrm{GUT}}$.
A priori, there are three sectors to be investigated i.e $\mathcal{A}_{12},\mathcal{A}_{13}$ and $\mathcal{A}_{23}$. However the (1,2) and (1,3) sectors are too constrained by the requirements that one should not get negative physical masses in the low scale spectrum and that loop corrections should not lead the CKM matrix to be outside the experimental range, therefore in the following only $A_{23}$ will be considered.
We implement SU(5)-like boundaries conditions i.e $M^2_\mathrm{Q}, M^2_\mathrm{U}$, $M^2_\mathrm{E}$ are unified in $M^2_{\mathbf{10}}$ and $M^2_\mathrm{L}$, $M^2_\mathrm{D}$ in $M^2_{\bar{\mathbf{5}}}$.
We also choose for simplicity, at the GUT scale, a common Higgs mass i.e $M_\mathrm{H} \equiv M_\mathrm{Hu}=M_\mathrm{Hd}$ and a common Gauginos mass noted $M_{1/2}$.
Finally we neglect all complex phases but the one introduced by the CKM matrix.
The benchmark point we take is given in table \ref{Num:Tab:BenchmarkPoint}.

\begin{table}
	\begin{center}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $\left(M^2_{\bold{10}}\right)_{i,j}$ & j=1       & j=2        & j=3      \\
				  \hline
				                                           i=1  & $(1000)^2$& 0          & 0        \\
				  \hline
				                           			       i=2  & 0         & $(3270)^2$ & $(557)^2$\\ 
				  \hline
				                            		       i=3  & 0         & $(557)^2$  & $(1550)^2$\\ 
				  \hline  
			\end{tabular}
			\hspace{0.5cm}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $\left(M^2_{\bold{\bar{5}}}\right)_{i,j}$ & j=1       & j=2        & j=3      \\
				  \hline
				                                           i=1  & $(860)^2$ & 0         & 0         \\
				  \hline
				                           			       i=2  & 0         & $(374)^2$ & 0         \\ 
				  \hline
				                            		       i=3  & 0         & 0         & $(412)^2$ \\ 
				  \hline  
			\end{tabular} 
			\vspace{0.5cm} \\
			\begin{tabular}{|l|l|l|l|} 
				
				  \hline
				  $a_u $ & j=1       & j=2       & j=3      \\
				  \hline
				   i=1   & 0         & 0         & 0         \\
				  \hline
				   i=2   & 0         & 0         & $(a_u)_{32}$\\ 
				  \hline
				   i=3   & 0         & $(a_u)_{23}$& -1500      \\ 
				  \hline  
			\end{tabular} 
			\hspace{0.5cm}
			\begin{tabular}{|l|l|l|l|} 
				  \hline
				  $a_d $ & j=1       & j=2       & j=3      \\
				  \hline
				   i=1   & 0         & 0         & 0         \\
				  \hline
				   i=2   & 0         & 0         & $(a_d)_{32}$\\ 
				  \hline
				   i=3   & 0         & $(a_d)_{23}$& 400      \\ 
				  \hline  
			\end{tabular}
			\hspace{0.5cm}
		\begin{tabular}{|l|} 
		 	\hline
		 	 $(M_{1∕2})^2=(1000)^2$ \\
		 	\hline 
			 $(M_{\mathrm{H}})^2=(1000)^2$  \\
			\hline 
			 $\mathrm{sign}(\mu)=+1$ \\
		 	\hline
		\end{tabular}
	\end{center}
\caption{GUT-defined soft breaking parameters: All masses and trilinears couplings are given in GeV. \label{Num:Tab:BenchmarkPoint}}
\end{table}

%Placing 1: Figures are at the end of the section but not on the same page!!%%%%%%%%%%%%%%%

	\begin{figure}[t]%\RawFloats
		\centering
	   \includegraphics[scale=0.60]{numerics_SU5/figures/SmallTanB/LowTanB.pdf}
	\caption{\label{Num:Pic:LowTanB}Low $\tan \beta$ regime: The thick black lines represents the isolines of $\mathcal{A}_{2,3}$ expressed in percentages of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} }$.  The  blue dashed lines and the red dashed-dotted lines  are the 2$\sigma$  exclusions bands on $\Delta M_\mathrm{Bs}$ and $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ respectively. The grey area represents the space which is excluded once all constraints are taken into account.}
	\end{figure}

		
	\begin{figure}[t]
		\centering
		\includegraphics[scale=0.60]{numerics_SU5/figures/HighTanB/HighTanB.pdf}
	\caption{\label{Num:Pic:HighTanB}High $\tan \beta$ regime: Same as figure \ref{Num:Pic:LowTanB}, the green dotted line is the lower bound of the 2$\sigma$ exclusion band on $\mathrm{BR}(b \rightarrow s \gamma)$.} 
	\end{figure}


We analyze the asymmetry in a low $\tan(\beta) \sim 10$ and a high $\tan(\beta) \sim 40$ regime.
In order to clarify which regions of parameter space is allowed experimentally, we also take into account several low energy constraints which we give hereafter with their 2$\sigma$ uncertainty:


\begin{tabular}{|l|}
\hline

	\item $\Delta M_{Bs} = (17.76 \pm 3.37)$ $\mathrm{ps}^{-1}$: The $B_s$ mesons oscillation frequency. 

\

\end{tabular}





\begin{itemize}
	\item $\Delta M_{Bs} = (17.76 \pm 3.37)$ $\mathrm{ps}^{-1}$: The $B_s$ mesons oscillation frequency. 
	\item $\epsilon_K/\epsilon_K^{\textrm{SM}} = (1 \pm 0.25)$: The ratio of the K mesons mixing parameter normalized to the value of the Standard Model. 
	\item $\mathrm{BR}(B^0_s\rightarrow \mu \mu) = (3.12 \pm 2.08)\times 10^{-9}$: The $B^0_s\rightarrow \mu \mu$ decay branching ratio.
	\item $\mathrm{BR}(b \rightarrow s \gamma) = (355 \pm 68)\times 10^{-6} $: The $b \rightarrow s \gamma$ decay branching ratio.
	\item $\mathrm{BR}(\tau \rightarrow \mu \gamma) < 4.5\times 10^{-8}$: The lepton number violating decay branching ratios of $\tau \rightarrow \mu \gamma$.
\end{itemize}
For each constraint, we make the quadratic sum of the experimental and theoretical errors.
We take the central values and experimental errors from the latest 2012 Heavy Flavor Collaboration Averaging Group report (see \cite{Amhis:2012bh}) and the theoretical errors from the following references (\cite{Misiak:2006zs}, \cite{Ball:2006xx}, \cite{Brod:2010mj}).
Moreover, we take into account the lightest higgs mass which we have assumed to correspond to the recently discovered scalar at the LHC. For its mass, we take the latest ATLAS central value 125.36$\pm$0.41(sys+stat) GeV see (\cite{Aad:2014aba}) quadratically summed with a theoretical error of $\pm$3 GeV.
The results are presented in fig \ref{Num:Pic:LowTanB} for the low $\tan \beta$ regime and in fig \ref{Num:Pic:HighTanB} for the high $\tan \beta$ regime.
On both figures, the thick black isolines represents the assymetry $\mathcal{A}_{2,3}$ expressed in percentage of $\sqrt{{\rm Tr}\mathcal{M}^2_{\tilde{u}}}$.
Note that we need to restrict this analysis to $ |(a_u)_{23}| < 600$ GeV, $|(a_d)_{23}| < 400$ GeV to avoid tachyons in the low scale spectrum, in particular the presence of tachyons in the spectrum depends critically on $(a_d)_{23}$.
We represent by colored lines the $2 \sigma$ exclusion band of the constraints when appropriate and by grey areas the excluded parameters space once all constraints are taken into account. 
In both regimes, $\mathrm{BR}(\tau \rightarrow \mu \gamma)$ never exceed the upper experimental value. We also manage to get a high and constant higgs mass ($m_h\sim$ 124 GeV) over the parameters range, especially due to the large negative top a-term ($a_t=-1500$ GeV).
In the low $\tan \beta$ regime, $\mathrm{BR}(b \rightarrow s \gamma)$ is kept within the $2\sigma$ exclusion band whereas this constraint is more severe for $\tan \beta \sim 40$, a part of the parameter space being excluded by it.
In the low $\tan \beta$ regime $\epsilon_K/\epsilon_K^{\textrm{SM}}$ is kept within the 1$\sigma$ band, due to the absence of complex phases in the soft terms, whereas in the high $\tan \beta$ regime, the supersymmetric contributions to $\epsilon_K$ are strongly suppressed, 
thus leading to $\epsilon_K/\epsilon_K^{\textrm{SM}} \sim 1$.
In any case, $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ and $\Delta M_{Bs}$ put the strongest constraints over the scanned parameter space (cf figs \ref{Num:Pic:LowTanB} and \ref{Num:Pic:HighTanB}).
To conclude, we see that the assymetry never exceed a few percents of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}}}$ which confirm that our master relation \ref{Eq:TrilinearUp} is indeed well preserved when running from $M_\textrm{GUT}$ down to $M_\textrm{SUSY}$ thus allowing to treat it as a theoretical uncertainty.






	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%Placing 2: Figures are gathered on the same page at the end of the section. Comes at the prize of half a page blank!%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%	\begin{figure}[p]%\RawFloats
%		\centering
%	   
%	   \includegraphics[scale=0.60]{numerics_SU5/figures/SmallTanB/LowTanB.pdf}
%	\caption{\label{Num:Pic:LowTanB}Low $\tan \beta$ regime: The thick black lines represents the isolines of $\mathcal{A}_{2,3}$ expressed in percentages of $\sqrt{{\rm Tr} \mathcal{M}^2_{\tilde{u}} }$.  The  blue dashed lines and the red dashed-dotted lines  are the 2$\sigma$  exclusions bands on $\Delta M_\mathrm{Bs}$ and $\mathrm{BR}(B^0_s\rightarrow \mu \mu)$ respectively. The grey area represents the space which is excluded once all constraints are taken into account.}
%	
%		\centering
%		
%		\includegraphics[scale=0.60]{numerics_SU5/figures/HighTanB/HighTanB.pdf}
%	\caption{\label{Num:Pic:HighTanB}High $\tan \beta$ regime: Same as figure \ref{Num:Pic:LowTanB}, the green dotted line is the lower bound of the 2$\sigma$ exclusion band on $\mathrm{BR}(b \rightarrow s \gamma)$.} 
%		
%	\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\FloatBarrier

==> stat/stat.tex <==


\section{ Statistical tools}

\label{se:stat}

We are going to use both frequentist and Bayesian statistics. 
When the $SU(5)$ test consists of a simple relation, for example among event rates, one can use a frequentist p-value test. 
This has the advantage of being  analytically computable in various limit cases. 
Otherwise, when a simple relation is not available, the standard method is to combine all datas in a  likelihood function. In our case, the likelihood will in principle depend on many theoretical parameters, which  possibly overcome the amount of constraints. In such ``partially-constrained'' problem, it is preferable to rely on Bayesian statistics, which are well-defined in this context. 


\subsection{Frequentist}

%We would like  to test a relation between some observable quantities $\mathcal{O}_i$, that can be put under the form \be r(\mathcal{O}_i)=0\,.
%\label{eq:r}

Assume one as a relation $R(\mathcal{O}_i)$ among observables quantities $\mathcal{O}_i$, that satisfies 
\be E[R(\mathcal{O}_i)]=0\,
\label{eq:r}
\ee 
whenever the $SU(5)$ hypothesis is verified. $E$ denotes the expectation operator.  We use a p-value test to quantify
whether or not the \textit{observed} value of $R$, denoted $\hat r$, is compatible with zero. This test is not trivial to perform in general, but simplifies whenever the probability density function (PDF) of $\hat r$ can be approximated by a half-normal law $\hat r \sim 2\mathcal{N}( r,\sigma)\theta(r)$ (see e.g. \cite{Cowan:2010js}), where $\theta$ is the unit step function.

In this case,  the  compatibility of $\hat r$ with the $r=0$ hypothesis can be expressed  in terms of a statistical significance as
\be
Z=\frac{|\hat r  |}{\sigma} \,. \label{eq:Z}
\ee
%\be
%Z=\Phi^{-1}\left(2\Phi\left( \frac{|\bar R|}{\sigma} \right)-1\right) \,. \label{eq:Z}
%\ee
Here  $Z=\Phi^{-1}(1-p)$ translates the p-value as a significance givens in term of standard Gaussian deviations. $\Phi$ is the standard Gaussian repartition function.  

For a given relation Eq.~\eqref{eq:r} and an hypothesized amount of data, one can evaluate the expected value of $\sigma$.  For a given significance $Z$, the quantity \be P_Z= Z\sigma \label{eq:PZ} \ee represents the \textit{expected precision} to which relation Eq.~\eqref{eq:r} can be tested. Throughout this paper we will systematically report $P_Z$ when a relation like Eq.~\eqref{eq:r} is available.




As an example, consider a relation like
\be
a X_1 = b X_2\,.
\ee
The $X_i$ are assumed to be normal variables, centered on $\mu_i$ and with variance $\sigma^2_i$.
One defines
\be
R=| a X_1 - b X_2 |\,.
\ee
 The PDF of $R$ takes then the form $f_R\sim 2\mathcal{N}( r,\sigma^2)\theta(r)$ where
\be
 r= a \mu_1 - b \mu_2 \,,
\ee
and the variance is 
\be
\sigma^2=a^2 \sigma^2_1+b^2 \sigma^2_2\,.
\ee
In order to compute the expected significance defined in Eq.~\eqref{eq:PZ}, one uses this $\sigma$ assuming that the $SU(5)$ hypothesis is true.  Note this implies $r=0$ by construction.

In practice it is useful to normalize $R$ such that $E[R]\in[0,1]$. The expected precision can then be expressed in percents. 
Concretely, the meaning of having $P_Z=20\%$ means that a violation of the relation $E[R]>20\%$ can be assessed with a $Z\sigma$ significance. 
The use of a normalized quantity is more convenient to interface the $SU(5)$ test with other studies -- either experimental or theoretical. Normalizing $R$ implies that one frequently encounters the random variable $|A-B|/(A+B)$, with $A$ and $B$ potentially correlated. One uses the notation $E[A]=\mu_A$, $E[B]=\mu_B$  $V[A]=\sigma_A^2$, $V[B]=\sigma_B^2$, $Cov[A,B]=\rho \sigma_A\sigma_B$.  The following relations are useful in order to derive the expected precision,
\be
E[A/B]\approx E[A]/E[B]\,,
\ee
\be
V[A/B]\approx \frac{1}{\mu_B^4}\bigg(\mu_A^2 \sigma_B^2+\mu_B^2 \sigma_A^2-2\rho \sigma_A \sigma_B \mu_A\mu_B  \bigg)
\ee
\be
V[(A-C)/(A+C)]\approx 
4\frac{\mu_A^2 \sigma^2_C+\mu_C^2 \sigma^2_A}{(\mu_A+\mu_C)^4} \approx 4V[(A)/(A+C)]~ \textrm{with}~ Cov[A,C]=0\,.
\ee
These approximations are in particular valid in the Gaussian limit, where a ratio of random variables is described by the Fieller-Hinkley distribution \cite{Hinkley}. For a large number of events $\mu_A\approx \sigma^2_A\approx N_A$ and similarly for $C$, one has 
\be
V[|N_A-N_C|/(N_A+N_C)]=\frac{N_A N_C}{(N_A + N_C)^3}\,.
\ee


%
% 
%As another example let us consider a relation of the form
%\be
%\frac{X_1}{X_2}=a \frac{X_3}{X_4}\,.
%\ee
%The PDF of a ratio $W=X_1/X_2$ is given by the  Fieller-Hinkley distribution \cite{Hinkley}. In the limit $\sigma_i\ll \mu_i$, it tends to a normal
%%\be
%%f(w)_W=\exp \bigg[ \frac{-(w-\mu_1/\mu_2)^2}{(2( \sigma_1^2/\mu_2^2+\mu_1^2\sigma_2^2/\mu_2^4 ))} \bigg]\,.
%%\ee
%\be
%f(w)_W \sim \mathcal{N}(\mu_1/\mu_2, (\mu_2^2\sigma_1^2+\mu_1^2\sigma_2^2)/\mu_2^4) 
%\ee
%
%The pdf of $R=|W_1-aW_2|$ is normal and obtained as above, with 
%\be
% r = \mu_1/\mu_2-a \mu_3/\mu_4\,,
%\ee
%\be
%\sigma^2= \bigg[\frac{\mu_2^2\sigma_1^2+\mu_1^2\sigma_2^2}{\mu_2^4}\bigg] 
%+ a^2     \bigg[\frac{\mu_4^2\sigma_3^2+\mu_3^2\sigma_4^2}{\mu_4^4}\bigg]\,.
%\ee
%This $\sigma$ can be then used in Eq.~\eqref{eq:PZ}.

\subsection{Bayesian}

\label{se:Stest}

 
 When a simple relation among observables is not available to test the $SU(5)$ hypothesis, the strategy by default is  to put  all available data in a likelihood function. The up-squark mass matrix and the rest of the SUSY parameters being in general only partially constrained by the data, Bayesian statistics have to be used.  
 In principle, performing a global Bayesian fit using the likelihood would provide all information available on the off-diagonal elements of $a_u$. However such a heavy task is actually unecessary for our purpose, as we are only interested in whether or not 
$a_u=a_u^t$. The rest of the parameters of the model does not interest us either. 
It is instead appropriate to use a Bayes factor to test the $SU(5)$  hypothesis. In our special case, the Bayes factor reduces to 
a so-called Savage-Dickey ratio test.  A short introduction to Bayesian hypothesis testing is included in App. \ref{se:Bayes}.  
  
  
%Moreover, in a scenario of  squark discovery, the pieces of information about the squark mass matrix would be gradually collected.
%In spite of the LHC expected performances and of possible progress in analysis techniques, obtaining enough information to fully 
%constrain the mass matrix during the LHC era is likely to be challenging. Most probably, the squark mass matrix would remain 
%only partially constrained during a long period.


  As we want to test whether or not the mass matrix has symmetric off-diagonal blocks, the two hypothesis we want to compare are 
\be
H_0 =\left\{ \mathcal{M}^2_{\tilde{u}} \not\in \hat{\mathbb{S}}_6 \right\}\, ,\quad H_1 =\left\{ \mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6 \right\}\,.
\ee
The Bayes factor Eq. \ref{eq:BF}  introduced is the tool that provides this comparison. 
One can naturally use the asymmetry  defined in (clarifier la ref une fois la section numerics ecrite) to characterize these properties. Our hypothesis then read     
\be
H_0 =\cup_i \left\{ \mathcal{A}_i\neq0 \right\}\, ,\quad H_1 =\cap_i\left\{ \mathcal{A}_i=0 \right\}\,.
\ee
Let us require that the prior on the mass matrix  satisfies the condition of factorisability necessary to simplify the Bayes factor into the SDDR. With this condition, the Bayes factor reduces to 
\be
S=S_{12}S_{13}S_{23}\,,\quad \label{eq:SDDR}
S_i=\left.\frac{p(\mathcal{A}_i|d)}{\int d\mathcal{A}_i\, p(\mathcal{A}_i|d))}\frac{1}{p(\mathcal{A}_i)}\right|_{\mathcal{A}_i=0}\,.
\ee
The $S$-test is the statistical test we are going to employ to study the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6$ hypothesis. 
For the upcoming discussions and examples below, it will be sufficient to focus on only one of the asymmetries $\mathcal{A}_i$ and the associated  test $S_i$. We  ommit the $i$ index from now on.
All discussions can be straightforwardly generalized to the case of several asymmetries as given  in Eq. \ref{eq:SDDR}. 

Following Jeffrey's scale, the values $S=3^{(-1)},12^{(-1)},150^{(-1)}$ correspond to weak, moderate, strong evidence for (against) the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6$ hypothesis. 
There is however a subtlety lying in the following case. If data indicates that $\mathcal{A}$ is compatible with zero, this can either point towards the 
$SU(5)$ hypothesis or indicate that the matrix elements are too small to be resolved by the data. 
 We thus define a complementary test in order to lift this degeneracy. The most natural way to proceed is to define the orthogonal quantity
\be
\tilde{ \mathcal{A}}=\ldots
\ee
\be
\tilde{ S}=\left.\frac{p(\tilde{\mathcal{A}}|d)}{\int d\tilde{\mathcal{A}}\, p(\tilde{\mathcal{A}}|d))}\frac{1}{p(\tilde{\mathcal{A}})}\right|_{\tilde{\mathcal{A}}=0}\,.
\ee 


Considering all possibilities for data, the $(S,\tilde{S})$ tests provide the following outputs. 
\begin{itemize}
\item If $S\ll1$, the test rules out the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6 $ hypothesis.
\item If $S\gg1$ and $\tilde S\ll1$, the test points out the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6 $ hypothesis.
\item If $S\gg1$ and $\tilde S\gg1$, the test is inconclusive in regard of the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6 $ hypothesis. Instead it points out the hypothesis of zero matrix elements $(\mathcal{M}^2_{\tilde u})_{26}=(\mathcal{M}^2_{\tilde u})_{35}=0$. 
More data may change the outcome.
\item  If $S\approx1$, or $S\gg1$ and $\tilde S\approx1$,  the test is inconclusive in regard of the $\mathcal{M}^2_{\tilde{u}} \in \hat{\mathbb{S}}_6 $ hypothesis. 
More data are necessary to change the outcome. 
\end{itemize}

The computation of the Bayes factor is in general a heavy task. However, it is rather simplified when it takes the form of a SDDR. 
We set up a computation based on a Markov Chain Monte Carlo (MCMC) algorithm. 
The principle is to define a  random walk whose density converges to the chosen target
distribution, presently the posterior, in the limit of many steps  (see \cite{Trotta:2008qt} for more about MCMCs).
The particularity of our present algorithm is that we are only interested in the posterior $p(\mathcal{A}|d)$ and the prior $p(\mathcal{A})$. 
We can thus fill in-flight  the histograms estimating these distributions, and easily check their convergence.
The particularity of this code is that it is  light and gets easily paralleled. 
 






